A Julia implementation of Algorithm NCL for constrained optimization

Algorithm NCL is designed for general smooth optimization problems where first and second derivatives are available, including problems whose constraints may not be linearly independent at a solution (i.e., do not satisfy the LICQ). It is equivalent to the LANCELOT augmented Lagrangian method, reformulated as a short sequence of nonlinearly constrained subproblems that can be solved efficiently by IPOPT and KNITRO, with warm starts on each subproblem. We give numerical results from a Julia implementation of Algorithm NCL on tax policy models that do not satisfy the LICQ, and on nonlinear least-squares problems and general problems from the CUTEst test set.

==> knitro_constrained_failures.tex <==
\begin{longtable}{lrrrccrrrrrrrl}
\caption{%
    \label{tab:knitro-cutest}
    \KNITRO results on CUTEst constrained problems.
}\\
\hline
name & nvar & ncon & \(f\)\hspace*{14pt} & \(\|\nabla L\|_2\) & \(\|c\|_2\) & \(t\)\hspace*{7pt} & iter & \#\(f\) & \#\(\nabla f\) & \#\(c\) & \#\(\nabla c\) & \#\(\nabla^2 L\) & status \\\hline
\endhead
\hline
\multicolumn{14}{r}{{\bfseries Continued on next page}}\\
\hline
\endfoot
\endlastfoot
CATENARY & \(  3003\) & \(  1000\) & \(-2.01\)e\(+10\) & \( 4.9\)e\(+00\) & \( 2.0\)e\(+09\) & \( 18.50\) & \(  2000\) & \(  7835\) & \(  2002\) & \(  7835\) & \(  2002\) & \(  2000\) & max\_iter \\
COSHFUN & \(  6001\) & \(  2000\) & \(-9.82\)e\(+17\) & \( 5.0\)e\(-01\) & \( 0.0\)e\(+00\) & \( 19.40\) & \(  2000\) & \(  2001\) & \(  2001\) & \(  2001\) & \(  2001\) & \(  2000\) & max\_iter \\
DRCAVTY1 & \(  4489\) & \(  3969\) & \( 0.00\)e\(+00\) & \( 0.0\)e\(+00\) & \( 2.2\)e\(-03\) & \( 456.00\) & \(  2000\) & \(  9191\) & \(  2002\) & \(  9191\) & \(  2002\) & \(  2000\) & max\_iter \\
EG3 & \( 10001\) & \( 20000\) & \( 5.11\)e\(+05\) & \( 2.0\)e\(+03\) & \( 3.3\)e\(-01\) & \( 7.18\) & \(    51\) & \(    55\) & \(    52\) & \(    55\) & \(    52\) & \(    52\) & infeasible \\
JUNKTURN & \( 10010\) & \(  7000\) & \( 1.78\)e\(-03\) & \( 1.0\)e\(-02\) & \( 6.4\)e\(-07\) & \( 123.00\) & \(  1913\) & \( 15051\) & \(  1915\) & \( 15051\) & \(  1915\) & \(  1914\) & unknown \\
LUKVLE11 & \(  9998\) & \(  6664\) & \( 5.12\)e\(+04\) & \( 5.1\)e\(+02\) & \( 4.1\)e\(-01\) & \( 86.50\) & \(  2000\) & \(  6945\) & \(  2001\) & \(  6945\) & \(  2001\) & \(  2000\) & max\_iter \\
LUKVLE17 & \(  9997\) & \(  7497\) & \( 3.22\)e\(+04\) & \( 1.8\)e\(-02\) & \( 9.9\)e\(-07\) & \( 47.00\) & \(  2000\) & \(  3190\) & \(  2001\) & \(  3190\) & \(  2001\) & \(  2000\) & max\_iter \\
LUKVLE18 & \(  9997\) & \(  7497\) & \( 1.12\)e\(+04\) & \( 4.0\)e\(+01\) & \( 2.5\)e\(-08\) & \( 83.90\) & \(  2000\) & \(  4190\) & \(  2001\) & \(  4190\) & \(  2001\) & \(  2000\) & max\_iter \\
ORTHRDS2 & \(  5003\) & \(  2500\) & \( 7.62\)e\(+02\) & \( 3.7\)e\(-01\) & \( 5.0\)e\(-13\) & \( 0.70\) & \(    42\) & \(    92\) & \(    43\) & \(    92\) & \(    43\) & \(    43\) & unknown \\\hline
\end{longtable}

